Resummed predictions for jet-resolution scales in multijet production in $e^+e^-$ annihilation

We present for the first time resummed predictions at NLO + NLL' accuracy for the Durham jet-resolution scales $y_{n,n+1}$ in multijet production in $e^+e^-$ collisions. Results are obtained using an implementation of the well known CAESAR formalism within the SHERPA framework. For the 4-, 5- and 6-jet resolutions we discuss in particular the impact of subleading colour contributions and compare to matrix-element plus parton-shower predictions from SHERPA and VINCIA.

==> changelog <==
Major:

	* Add LO+NLL' and NLL ratios to Fig. 5. and add
	"The lower panels show the corresponding ratios additionally at
	$\mathrm{LO+NLL}^\prime$ accuracy and for the resummation without
	any matching."
	to caption
	* Add discussion of unmatched ratios to main text (see todo)
	* Fig. 2 -> y-axis to linear and adjust caption
	* Add discussion of subleading contributions (see 2 todos),
	including a new figure for the F-function for y_23

Minor:
	* Fix label on lilac line in Fig. 4.
	* Add Ref. [56] to arXiv:2001.11492
	* Fix missing bibliography entry for Ref. [49]
	* Fix typo in Eq. (12)
	* Fix typo in definition of rapidity below Eq. 12
	* Fix typo just before Eq. (14)
	* Fix typo p5, 2nd to last line
	* Add acknowledgement of CTP's scholarships

